Transfer Learning with Bellwethers to find Good Configurations

As software systems grow in complexity, the space of possible configurations grows exponentially. Within this increasing complexity, developers, maintainers, and users cannot keep track of the interactions between all the various configuration options. Finding the optimally performing configuration of a software system for a given setting is challenging. Recent approaches address this challenge by learning performance models based on a sample set of configurations. However, collecting enough data on enough sample configurations can be very expensive since each such sample requires configuring, compiling and executing the entire system against a complex test suite. The central insight of this paper is that choosing a suitable source (a.k.a. "bellwether") to learn from, plus a simple transfer learning scheme will often outperform much more complex transfer learning methods. Using this insight, this paper proposes BEETLE, a novel bellwether based transfer learning scheme, which can identify a suitable source and use it to find near-optimal configurations of a software system. BEETLE significantly reduces the cost (in terms of the number of measurements of sample configuration) to build performance models. We evaluate our approach with 61 scenarios based on 5 software systems and demonstrate that BEETLE is beneficial in all cases. This approach offers a new highwater mark in configuring software systems. Specifically, BEETLE can find configurations that are as good or better as those found by anything else while requiring only 1/7th of the evaluations needed by the state-of-the-art.

==> tex/approach1.tex <==
\begin{figure*}[htbp]
\centering
\begin{subfigure}[t]{0.45\linewidth}
\centering
\textbf{Pick Bellwether Environment}\\[0.5cm]
\includegraphics[width=\linewidth]{figures/source_target.png}
\end{subfigure}\hspace{5pt}
\begin{subfigure}[t]{0.5\linewidth}
\hspace{0.4\linewidth}\textbf{Pseudocode}
\small
\begin{lstlisting}[xleftmargin=8.0ex,mathescape,frame=none,numbers=left]
def FindBellwether(sources, step_size, budget, thres, lives): 
  while lives or cost > budget:
    "Sample configurations"
    sampled = list()
    for source in sources:
      sampled += source.sample(step_size)
    "Get cost"
    cost = get_cost(sampled)
    "Evaluate pair-wise performances"
    perf = get_perf(sampled)
    "Remove non-bellwether environments"
    sources = remove_non_bellwethers(sources, perf, thres)
    "Loose life if no sources are removed"
    if prev == len(sources): lives -= 1
    "Return a bellwether"
  return sources[argmin(perf)]
\end{lstlisting}
\end{subfigure}\\[0.4cm]
\begin{subfigure}[t]{0.5\linewidth}
\centering
\textbf{Transfer Learning with Bellwether Environment}\\
\includegraphics[width=0.85\linewidth]{figures/bellwether-transfer.png}
\end{subfigure}~~%
\begin{subfigure}[t]{0.5\linewidth}
\vspace{0.4cm}
\hspace{0.4\linewidth}\textbf{Pseudocode}\\[-0.3cm]
\small
\begin{lstlisting}[xleftmargin=5.0ex,mathescape,frame=none,numbers=left]
def BEETLE(sources, target, budget): 
    "Find the bellwether environment"
    bellwether = FindBellwether(sources, step_size, budget, thres, lives)
    "Sample the bellwether source to fit budget"
    b_some = bellwether.sample(budget)
    "Train a prediction model with the bellwether"
    prediction_model = regTree.train(b_some)
    predicted = prediction_model.test(target.indep)
    return target[argmin(predicted)]
\end{lstlisting}
\end{subfigure}	
\caption{{\small This figure demonstrates the two key aspects of our proposed approach for transfer learning (a)~how to pick the bellwether environment; (b)~How to construct a  transfer learner with the bellwether environment. A visual intuition of each of the two methods is presented on the left and the corresponding pseudocode are presented on the right.}}
\label{fig:approach}
\end{figure*}
